Averaging Bias: Human Faithfulness Annotations are not Locally Faithful

Evaluation of faithfulness of text summarization treats a model generated summary as faithful only if every of its sentences is supported by the source document: a strict conjunctive rule under which a single unsupported sentence makes the whole summary unfaithful. Yet most faithfulness benchmarks collect only one global human annotation label per summary. We ask whether such global human labels actually implement the conjunctive rule. We hypothesize that annotators may accept a summary as faithful when most sentences are faithful, not only when all are faithful. To test our hypothesis, we use five large language model (LLM) judges as per-sentence raters across four widely used faithfulness benchmarks. We find that global human labels correlate better with the average of per-sentence LLM judgments than with the implementation of the strict conjunctive rule. A manual review confirms that a substantial fraction of summaries labeled faithful by humans contain genuine local factual errors. We call this tendency Averaging Bias. Our results reveal that human labels on widely used faithfulness benchmarks contain measurable Averaging Bias, calling for carefully structured designs for trustworthy human annotations

==> tables/main.tex <==
% Auto-generated from results/meta_eval_summary.*.csv
% Overall rows only; hard sentence labels; Pearson/Spearman/Kendall/ROC-AUC.
\begin{table*}[t!]
\centering
\small
\begin{tabular}{llrrrr}
\hline
Model & Aggregation & Pearson $r$ & Spearman $\rho$ & Kendall $\tau$ & ROC-AUC\\
\hline
\multicolumn{6}{c}{\textbf{AggreFact-CNN}}\\
\hline
Qwen3-4B & min & +0.224 & +0.224 & +0.224 & +0.572\\
Qwen3-4B & mean & +0.244 & +0.225 & +0.223 & +0.573\\
Qwen3-4B & max & +0.087 & +0.087 & +0.087 & +0.504\\
Qwen3-8B & min & +0.274 & +0.274 & +0.274 & +0.629\\
Qwen3-8B & mean & +0.272 & +0.277 & +0.272 & +0.631\\
Qwen3-8B & max & +0.087 & +0.087 & +0.087 & +0.504\\
Qwen3-32B & min & +0.386 & +0.386 & +0.386 & +0.673\\
Qwen3-32B & mean & +0.409 & +0.392 & +0.386 & +0.676\\
Qwen3-32B & max & +0.087 & +0.087 & +0.087 & +0.504\\
Llama-3.1-8B & min & +0.250 & +0.250 & +0.250 & +0.627\\
Llama-3.1-8B & mean & +0.234 & +0.250 & +0.244 & +0.627\\
Llama-3.1-8B & max & -0.011 & -0.011 & -0.011 & +0.499\\
OLMo-3-7B & min & +0.197 & +0.197 & +0.197 & +0.650\\
OLMo-3-7B & mean & +0.211 & +0.205 & +0.191 & +0.661\\
OLMo-3-7B & max & +0.104 & +0.104 & +0.104 & +0.518\\
\hline
\multicolumn{6}{c}{\textbf{AggreFact-other}}\\
\hline
Qwen3-4B & min & +0.065 & +0.065 & +0.065 & +0.536\\
Qwen3-4B & mean & +0.162 & +0.160 & +0.150 & +0.615\\
Qwen3-4B & max & +0.205 & +0.205 & +0.205 & +0.622\\
Qwen3-8B & min & +0.101 & +0.101 & +0.101 & +0.553\\
Qwen3-8B & mean & +0.191 & +0.192 & +0.180 & +0.638\\
Qwen3-8B & max & +0.211 & +0.211 & +0.211 & +0.634\\
Qwen3-32B & min & +0.179 & +0.179 & +0.179 & +0.605\\
Qwen3-32B & mean & +0.215 & +0.216 & +0.202 & +0.657\\
Qwen3-32B & max & +0.189 & +0.189 & +0.189 & +0.617\\
Llama-3.1-8B & min & +0.131 & +0.131 & +0.131 & +0.580\\
Llama-3.1-8B & mean & +0.148 & +0.134 & +0.126 & +0.596\\
Llama-3.1-8B & max & +0.136 & +0.136 & +0.136 & +0.571\\
OLMo-3-7B & min & +0.141 & +0.141 & +0.141 & +0.582\\
OLMo-3-7B & mean & +0.167 & +0.172 & +0.161 & +0.625\\
OLMo-3-7B & max & +0.142 & +0.142 & +0.142 & +0.590\\
\hline
\multicolumn{6}{c}{\textbf{DiverSumm}}\\
\hline
Qwen3-4B & min & +0.357 & +0.357 & +0.357 & +0.685\\
Qwen3-4B & mean & +0.112 & +0.264 & +0.232 & +0.653\\
Qwen3-4B & max & -0.103 & -0.103 & -0.103 & +0.463\\
Qwen3-8B & min & +0.311 & +0.311 & +0.311 & +0.649\\
Qwen3-8B & mean & +0.182 & +0.258 & +0.222 & +0.654\\
Qwen3-8B & max & -0.061 & -0.061 & -0.061 & +0.477\\
Qwen3-32B & min & +0.324 & +0.324 & +0.324 & +0.656\\
Qwen3-32B & mean & +0.154 & +0.256 & +0.220 & +0.653\\
Qwen3-32B & max & -0.090 & -0.090 & -0.090 & +0.467\\
Llama-3.1-8B & min & +0.229 & +0.229 & +0.229 & +0.619\\
Llama-3.1-8B & mean & +0.017 & +0.164 & +0.149 & +0.591\\
Llama-3.1-8B & max & -0.119 & -0.119 & -0.119 & +0.459\\
OLMo-3-7B & min & +0.117 & +0.117 & +0.117 & +0.547\\
OLMo-3-7B & mean & +0.131 & +0.157 & +0.132 & +0.594\\
OLMo-3-7B & max & -0.070 & -0.070 & -0.070 & +0.473\\
\hline
\multicolumn{6}{c}{\textbf{HaluEval}}\\
\hline
Qwen3-32B & min & +0.394 & +0.394 & +0.394 & +0.697\\
Qwen3-32B & mean & +0.472 & +0.469 & +0.421 & +0.755\\
Qwen3-32B & max & +0.276 & +0.276 & +0.276 & +0.575\\
\hline
\end{tabular}
\caption{Overall correlations between aggregated sentence-level LLM faithfulness scores and human summary labels. Only the hard sentence-label setting is shown. For each dataset and model, rows report the three core aggregation functions: minimum, mean, and maximum.}
\label{tab:overall-pearson-main}
\end{table*}

